Optimal Lower Bound on the Least Singular Value of the Shifted Ginibre Ensemble

We consider the least singular value of a large random matrix with real or complex i.i.d. Gaussian entries shifted by a constant $z\in\mathbb{C}$. We prove an optimal lower tail estimate on this singular value in the critical regime where $z$ is around the spectral edge thus improving the classical bound of [Sankar, Spielman, Teng, 2006] in the edge regime. Lacking Br\'ezin-Hikami formulas in the real case, we rely on the superbosonization formula [Littelmann, Sommers, Zirnbauer, 2008].

==> packages_and_notation.tex <==
%
%
\usepackage{graphicx} 
\usepackage{color,bm} %
\usepackage{amsmath,amssymb,amsthm,mathrsfs,amsfonts,dsfont,braket} 
\usepackage{listings}
\usepackage[shortlabels]{enumitem} 
\usepackage{booktabs,changepage}
\usepackage{xspace,afterpage} 
\usepackage[printonlyused,withpage]{acronym} 
\usepackage{rotating} 
\usepackage{mathrsfs} 
\usepackage{hyperref}
\usepackage{etoolbox}
\usepackage{asymptote}
\patchcmd{\abstract}{\scshape\abstractname}{\textbf{\abstractname}}{}{}
\usepackage[dvipsnames]{xcolor}
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\makeatletter
%
\setcounter{tocdepth}{3}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
\addtolength{\textheight}{-\baselineskip}
\addtolength{\footskip}{\baselineskip}
\usepackage{dsfont,xstring}
\RequirePackage{setspace}
\usepackage{pgfplots} 
\pgfplotsset{compat=newest} 
\usepgfplotslibrary{fillbetween,colorbrewer}
%
%
%
%
%
  %
%
%
%
%
%
\hypersetup{colorlinks, breaklinks, linkcolor=MidnightBlue,citecolor=BrickRed,filecolor=black}%
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section}
\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{(\Alph{assumption})}

\makeatletter
\def\section{\@startsection{section}{1}%
\z@{.7\linespacing\@plus\linespacing}{.5\linespacing}%
{\normalfont\bfseries\centering}}
\makeatother

\newcommand{\ii}{\mathrm{i}}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\lstset{
  basicstyle=\ttfamily\small,
  basewidth=0.55em,
  showstringspaces=false,
  numbers=left,
  numberstyle=\tiny,
  numbersep=2.5pt,
  keywordstyle=\bfseries\ttfamily,
  breaklines=true
}
\lstnewenvironment{pseudoc}{\lstset{frame=lines,language=C,mathescape=true}}{}
\lstnewenvironment{logs}{\lstset{frame=lines,basicstyle=\footnotesize\ttfamily,numbers=none}}{}
\lstnewenvironment{cc}{\lstset{frame=lines,language=C}}{}
\lstnewenvironment{c64}{\lstset{backgroundcolor=\color{c64},basewidth=0.65em,basicstyle=\commodoreface\color{c64light},numbers=none,framerule=10pt,rulecolor=\color{c64light},frame=tb,framexbottommargin=30pt}}{}
\lstnewenvironment{html}{\lstset{frame=lines,language=html,numbers=none}}{}
\lstnewenvironment{pseudo}{\lstset{frame=lines,mathescape=true,morekeywords={learn_string_domain, save_model}}}{}
\lstnewenvironment{pseudoctiny}{\lstset{language=C,mathescape=true,basicstyle=\tiny\sffamily}}{}
\lstnewenvironment{cctiny}{\lstset{language=C,basicstyle=\tiny\sffamily}}{}
\lstnewenvironment{pseudotiny}{\lstset{mathescape=true,basicstyle=\tiny\sffamily}}{}
\pgfplotsset{plot coordinates/math parser=false} 
\newtheorem*{genericthm*}{Assumption \ref{assumption correlations}'}
\newtheorem*{assCD}{Assumption (CD)}

\newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3}}
\theoremstyle{named}
\newtheorem*{namedtheorem}{Theorem}
\newlength\figureheight
\newlength\figurewidth
%
\usepackage{grffile}
%
\renewcommand*{\acffont}[1]{{\normalsize\itshape #1}}
\renewcommand*{\acfsfont}[1]{{\normalsize\upshape #1}} 
\usetikzlibrary{plotmarks}
\usetikzlibrary{calc,decorations.markings}

%
%

\newcommand{\inD}[1]{\quad\text{in}\quad\DD_{#1}^\delta}
\newcommand{\inG}[1]{\quad\text{in}\quad\GG_{#1}^\delta}

%
\usepackage{authblk}
\usepackage{subcaption,amsaddr}
\newcommand{\As}{\mathcal{A}}
\newcommand{\1}{\mathds{1}}
\newcommand{\R}{\mathbb{R}}  %
\ifdefined\C\renewcommand{\C}{\mathbb{C}}\else\newcommand{\C}{\mathbb{C}}\fi %
\newcommand{\N}{\mathbb{N}}  %
\newcommand{\cE}{\mathcal{E}}  %
\newcommand{\cG}{\mathcal{G}}  %

\newcommand{\Hi}{\mathcal{H}}  %
\newcommand{\HC}{\mathbb{H}}  %
\newcommand{\BV}{BV}  %
\newcommand{\deq}{%
  \mathrel{\vbox{\offinterlineskip\ialign{%
    \hfil##\hfil\cr
    \(\scriptscriptstyle d\)\cr
    \noalign{\kern.1ex}
    \(=\)\cr
}}}}
\renewcommand{\star}{\(^*\)}
\newcommand{\Z}{\mathbb{Z}}  %
\newcommand{\DD}{\mathbb{D}}  %
\newcommand{\GG}{\mathbb{G}}  %
\newcommand{\CC}{\mathcal{C}}
\newcommand{\sa}{\mathrm{sa}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\GOE}{\mathrm{GOE}}
\newcommand{\GUE}{\mathrm{GUE}}

\newcommand{\hs}{\mathrm{hs}}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}

\newcommand{\vx}{\mathbf{x}}
\newcommand{\HS}{\mathrm{hs}}

\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\Tuple}[1]{
\left(\,
\StrSubstitute{#1}{|}{\;\middle\vert\;}[\temp]%
\temp
\,\right)
}
\newcommand{\tuple}[1]{
(\,
\StrSubstitute{#1}{|}{\;\vert\;}[\temp]%
\temp
\,)
}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\NN}{\mathcal{N}}

\newcommand{\vu}{\mathbf{u}}
\newcommand{\cI}{\mathcal{I}}

\newcommand{\vv}{\mathbf{v}}
\newcommand{\vm}{\mathbf{m}}
\newcommand{\BB}{\mathcal{B}}

\renewcommand{\SS}{\mathcal{S}}

\newcommand{\Q}{\mathbb{Q}}  %
\newcommand{\K}{\mathbb{K}} %
\newcommand{\LO}{\mathcal{L}} %
\newcommand{\cP}{\mathcal{P}} %
\newcommand{\cR}{\mathcal{R}} %
\newcommand{\cJ}{\mathcal{J}} %
\newcommand{\cC}{\mathcal{C}} %

\newcommand{\cQ}{\mathcal{Q}} %
\newcommand{\Sp}{\mathbf{S}} %
\newcommand{\ed}{\mathfrak{e}}
\newcommand{\BO}{\mathcal{B}} %
\newcommand{\DO}{\mathcal{D}} %
\newenvironment{smatrix}{\left(\begin{smallmatrix}}{\end{smallmatrix}\right)}
\renewcommand{\L}{\mathcal{L}} %

\newcommand{\FO}{\mathcal{F}} %
\newcommand{\KO}{\mathcal{K}} %
\newcommand{\landauo}[1]{\scriptstyle\mathcal{O}\textstyle\left(#1\right)} 
\newcommand{\landauOsubscript}[2]{\mathcal{O}_{#1}\left(#2\right)} 
\newcommand{\landauOstd}[1]{\mathcal{O}\left(#1\right)} 
\newcommand{\landauO}[2][]{\mathcal{O}_{#1}\left(#2\right)}
\newcommand{\stO}[1]{\mathcal{O}_\prec\left(#1\right)} 
 
\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt\hbox{\scriptsize.}\hbox{\scriptsize.}}}=}
\newcommand*{\defqe}{=\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt\hbox{\scriptsize.}\hbox{\scriptsize.}}}}                     
\newcommand{\norms}[2][0]{%
  \ifcase#1\relax
    \lVert #2\rVert\or         %
    \big\lVert #2\big\rVert\or   %
    \Big\lVert #2\Big\rVert\or   %
    \bigg\lVert #2\bigg\rVert\or  %
    \Bigg\lVert #2\Bigg\rVert\or     %
    \left\lVert #2\right\rVert
  \fi
} 
\makeatletter
\def\norm{\@ifnextchar[{\@normwith}{\@normwithout}}
\def\@normwith[#1]#2{\norms[#1]{#2}}
\def\@normwithout#1{\norms[5]{#1}}
\makeatother

\newcommand{\tnorms}[2][0]{%
  \ifcase#1\relax
    \lvert\kern-0.25ex\lvert\kern-0.25ex\lvert #2 \rvert\kern-0.25ex\rvert\kern-0.25ex\rvert\or %
    \big\lvert\kern-0.25ex\big\lvert\kern-0.25ex\big\lvert #2 \big\rvert\kern-0.25ex\big\rvert\kern-0.25ex\big\rvert\or   %
    \Big\lvert\kern-0.25ex\Big\lvert\kern-0.25ex\Big\lvert #2 \Big\rvert\kern-0.25ex\Big\rvert\kern-0.25ex\Big\rvert\or   %
    \bigg\lvert\kern-0.25ex\bigg\lvert\kern-0.25ex\bigg\lvert #2 \bigg\rvert\kern-0.25ex\bigg\rvert\kern-0.25ex\bigg\rvert\or   %
    \Bigg\lvert\kern-0.25ex\Bigg\lvert\kern-0.25ex\Bigg\lvert #2 \Bigg\rvert\kern-0.25ex\Bigg\rvert\kern-0.25ex\Bigg\rvert\or   %
    \left\lvert\kern-0.25ex\left\lvert\kern-0.25ex\left\lvert #2 \right\rvert\kern-0.25ex\right\rvert\kern-0.25ex\right\rvert
  \fi
} 
\makeatletter
\def\tnorm{\@ifnextchar[{\@tnormwith}{\@tnormwithout}}
\def\@tnormwith[#1]#2{\tnorms[#1]{#2}}
\def\@tnormwithout#1{\tnorms[5]{#1}}
\makeatother

\newcommand{\abss}[2][0]{%
  \ifcase#1\relax
    \lvert #2\rvert\or         %
    \big\lvert #2\big\rvert\or   %
    \Big\lvert #2\Big\rvert\or   %
    \bigg\lvert #2\bigg\rvert\or  %
    \Bigg\lvert #2\Bigg\rvert\or     %
    \left\lvert #2\right\rvert
  \fi
} 
\makeatletter
\def\abs{\@ifnextchar[{\@abswith}{\@abswithout}}
\def\@abswith[#1]#2{\abss[#1]{#2}}
\def\@abswithout#1{\abss[5]{#1}}
\makeatother

\providecommand{\maxnorm}[1]{\left\lVert#1\right\lVert_{\text{max}}} %
\providecommand{\braket}[1]{\left\langle#1\right\rangle} %
\providecommand{\Cov}[1]{\mathbf{Cov}\left(#1\right)} %
\providecommand{\CovBig}[1]{\mathbf{Cov}\Big(#1\Big)} %
\providecommand{\Covbig}[1]{\mathbf{Cov}\big(#1\big)} %

\providecommand{\floor}[1]{\lfloor#1\rfloor} %

\renewcommand{\implies}{\Rightarrow}

\DeclareMathOperator{\esssup}{ess~sup}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\erf}{erf}

\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\Rai}{rai}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\interior}{int}

%

\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\cone}{cone}

\DeclareMathOperator{\Ran}{Ran}
\DeclareMathOperator{\dlim}{d-lim}
\DeclareMathOperator{\Gin}{Gin}


\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Endsa}{End_\mathrm{sa}}
\DeclareMathOperator{\sdet}{SDet}
\DeclareMathOperator{\sTr}{STr}

\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Val}{Val}
\DeclareMathOperator{\SVal}{SVal}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\F}{\mathbb{F}}

\newcommand{\sS}{\mathsf{S}}
\newcommand{\sSc}{\mathsf{S}_\mathrm{c}}
\newcommand{\sSd}{\mathsf{S}_\mathrm{d}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sPc}{\mathsf{P}_\mathrm{c}}
\newcommand{\sPd}{\mathsf{P}_\mathrm{d}}

\newcommand{\cPu}{\mathcal{P}_\mathrm{u}}
\newcommand{\cPl}{\mathcal{P}_\mathrm{l}}

\newcommand{\sM}{\mathsf{M}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cT}{\mathcal{T}}


\newcommand{\cM}{\mathcal{M}}
\newcommand{\cU}{\mathcal{U}}


\newcommand{\cF}{\mathcal{F}}
\newcommand{\cW}{\mathcal{W}}

\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\sgn}{sgn}

\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\maxroot}{maxroot}
\DeclareMathOperator{\arctanh}{arctanh}


\DeclareMathOperator{\E}{\mathbf{E}}
\DeclareMathOperator{\Var}{\mathbf{Var}}
%

%
\renewcommand{\P}{\mathbf{P}}
%
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\wlim}{w-lim}


\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\graph}{Gr} %
\DeclareMathOperator{\dist}{dist} %
\newcommand{\ba}{{\mathbf a}}
\newcommand\restr[2]{{%
  \left.\kern-\nulldelimiterspace %
  #1 %
  \vphantom{\big|} %
  \right|_{#2} %
  }}
\makeatletter
\providecommand*{\diff}%
        {\@ifnextchar^{\DIfF}{\DIfF^{}}}
\def\DIfF^#1{%
        \mathop{\mathrm{\mathstrut d}}%
                \nolimits^{#1}\gobblespace
}
\def\gobblespace{%
        \futurelet\diffarg\opspace}
\def\opspace{\let\DiffSpace\! \ifx\diffarg(\let\DiffSpace\relax\else\ifx\diffarg\let\DiffSpace\relax\else\ifx\diffarg\{\let\DiffSpace\relax\fi\fi\fi\DiffSpace}  
\newcommand{\cor}{\color{red}}
\newcommand{\cred}[1]{{\color{red} #1}}
\newcommand{\cblue}[1]{{\color{blue} #1}}
\newcommand{\cob}{\color{blue}}
\newcommand{\nc}{\normalcolor}
\newcommand{\ov}{\overline}


\usepackage[style=phys,giveninits=true,url=false,doi=false,isbn=false,eprint=true,datamodel=mrnumber,sorting=nty,maxcitenames=4,maxbibnames=99,backref=false,block=space,backend=biber]{biblatex}
\renewbibmacro{in:}{}
\DefineBibliographyStrings{english}{%
  backrefpage = {see p.~},%
  backrefpages = {see pp.},%
}
\bibliography{references}
\ExecuteBibliographyOptions{eprint=true}
\DeclareFieldFormat[article]{title}{\emph{#1}} 
\DeclareFieldFormat{mrnumber}{%
  \ifhyperref
    {\href{http://www.ams.org/mathscinet-getitem?mr=#1}{\nolinkurl{MR#1}}}
    {\nolinkurl{#1}}}
\DeclareFieldFormat{pmid}{%
  \ifhyperref
    {\href{https://www.ncbi.nlm.nih.gov/pubmed/#1}{\nolinkurl{PMID#1}}}
    {\nolinkurl{#1}}}
\DeclareFieldFormat{eprint}{%
  \ifhyperref
    {\href{https://arxiv.org/abs/#1}{\nolinkurl{arXiv:#1}}}
    {\nolinkurl{#1}}}
\renewbibmacro*{doi+eprint+url}{%
  \iftoggle{bbx:doi}
    {\printfield{doi}}
    {}%
  \newunit\newblock
  \printfield{mrnumber}%
  \newunit\newblock
  \printfield{pmid}%
  \newunit\newblock
  \printfield{eprint}%
  %
  %
  %
  %
  \newunit\newblock
  \iftoggle{bbx:url}
    {\usebibmacro{url+urldate}}
    {}}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\begin{asydef}
import graph;
import contour;
import palette;
size(12cm,6cm,IgnoreAspect);
int N=200;
int Levels=10;
pen[] Palette=Gradient(Levels,RGB(100,100,255),RGB(255,100,100));
defaultpen(fontsize(8pt));
\end{asydef}
